A mirror inertial forward-reflected-backward splitting: Global convergence and linesearch extension beyond convexity and Lipschitz smoothness

This work investigates a Bregman and inertial extension of the forward-reflected-backward algorithm [Y. Malitsky and M. Tam, SIAM J. Optim., 30 (2020), pp. 1451--1472] applied to structured nonconvex minimization problems under relative smoothness. To this end, the proposed algorithm hinges on two key features: taking inertial steps in the dual space, and allowing for possibly negative inertial values. Our analysis begins with studying an associated envelope function that takes inertial terms into account through a novel product space formulation. Such construction substantially differs from similar objects in the literature and could offer new insights for extensions of splitting algorithms. Global convergence and rates are obtained by appealing to the generalized concave Kurdyka-Lojasiewicz (KL) property, which allows us to describe a sharp upper bound on the total length of iterates. Finally, a linesearch extension is given to enhance the proposed method.

==> TeX/Text/Preliminaries_GCKL.tex <==
{\red\bf ZW: TODO: 1. Simplify Title {\blue(AT: change OK?)}. 2. Add comment if space permits}

{\blue\bf AT: Isn't it too advanced to present here? Perhaps more fit in \cref{sec:convergence}, since it is used there}

In this section we introduce a key concept that will be fundamental in \cref{sec:convergence}. For $\eta\in(0,\infty]$, denote by $\Psi_\eta$ the class of functions $\psi:[0,\eta)\rightarrow\R_+$ satisfying the following: (i) $\psi(t)$ is right-continuous at $t=0$ with $\psi(0)=0$; (ii) $\psi$ is strictly increasing on $[0,\eta)$. 

\begin{definition}\emph{\cite[Definition 5]{wang2022exact}}\label{def: GCKL} Let $f:\R^n\rightarrow\overline{\R}$
	be proper and lsc.  Let $\bar{x}\in\dom\partial f$ and $\mu\in\R$, and
	let $V\subseteq\dom\partial f$ be a nonempty subset.
	\begin{enumerate}
		\item We say that $f$ has the pointwise generalized concave Kurdyka-\L ojasiewicz~(KL) property at $\bar{x}\in\dom\partial f$, if there exist neighborhood $U\ni\bar{x}$, $\eta\in(0,\infty]$ and concave $\psi\in\Psi_\eta$, such that for all $x\in U\cap[0<f-f(\bar{x})<\eta]$,
		\begin{equation*}\label{g-concave KL inequality}
			\psi^\prime_-\big(f(x)-f(\bar{x})\big)\cdot\dist\big(0,\partial f(x)\big)\geq1,
		\end{equation*}
		where $\psi_-^\prime$ denotes the left derivative. Moreover, $f$ is a generalized concave KL function if it has the generalized concave KL property at every $x\in\dom\partial f$.
		\item Suppose that $f(x)=\mu$ on $V$. We say $f$ has the setwise\footnote{We shall omit adjectives ``pointwise'' and ``setwise'' whenever there is no ambiguity.} generalized concave KL property on $V$ if there exist $U\supset V$, $\eta\in(0,\infty]$ and concave $\psi\in\Psi_\eta$ such that for every $x\in U\cap[0<f-\mu<\eta]$,
		\begin{equation*}\label{uniform g-concave KL inequality}
			\psi^\prime_-\big(f(x)-\mu\big)\cdot\dist\big(0,\partial f(x)\big)\geq1.
		\end{equation*}
	\end{enumerate}
\end{definition}

For subset $\Omega\subseteq\R^n$, define $(\forall \varepsilon>0)$ $\Omega_\varepsilon=\{x\in\R^n:\dist(x,\Omega)<\varepsilon\}$. 
\begin{lemma}\label{lemma: Uniformize GCKL}\emph{\cite[Lemma 4.4]{wang2022exact}} Let $f:\R^n\rightarrow\overline{\R}$ be proper lsc and let $\mu\in\R$. Let $\Omega\subseteq\dom\partial f$ be a nonempty compact set on which $f(x)=\mu$ for all $x\in\Omega$. Then the following hold:
	\begin{enumerate}
		\item Suppose that $f$ satisfies the pointwise generalized concave KL property at each $x\in\Omega$. Then there exist $\varepsilon>0,\eta\in(0,\infty]$ and $\psi\in\Psi_\eta$ such that $f$ has the setwise generalized concave KL property on $\Omega$ with respect to $U=\Omega_\varepsilon$, $\eta$ and $\psi$.
		
		\item\label{uniformize exact modulus} Set $U=\Omega_\varepsilon$ and define $h:(0,\eta)\rightarrow\R_+$ by \[h(s)=\sup\big\{\dist^{-1}\left(0,\partial f(x)\right):x\in U\cap[s\leq f-\mu<\eta]\big\}.\]
		Then the function $\tilde{\psi}:[0,\eta)\rightarrow\R_+$ defined by \((\forall 0<t<\eta)~\tilde\psi(t)=\int_0^th(s)ds\) with \(\tilde{\psi}(0)=0\) is well defined and belongs to $\Psi_\eta$. The function $f$ has the setwise generalized concave KL property on $\Omega$ with respect to $U$, $\eta$ and $\tilde{\psi}$. Moreover,
		\[
		\tilde{\psi}
		{}={}
		\inf\left\{
		\psi\in\Psi_\eta
		\,\Big|\,
		\text{\begin{tabular}{@{}c@{}}%
				\(\psi\) is a concave desingularizing function\\
				of $f$ on $\Omega$ with respect to $U$ and $\eta$
		\end{tabular}}
		\right\}.
		\]
	\end{enumerate}
	We say that $\tilde{\psi}$ is the exact modulus of the setwise generalized concave KL property of \(f\) on \(\Omega\) with respect to $U$ and $\eta$.
\end{lemma}

